Attaining Equilibria Using Control Sets

Many interactions result in a socially suboptimal equilibrium, or in a non-equilibrium state, from which arriving at an equilibrium through simple dynamics can be impossible of too long. Aiming to achieve a certain equilibrium, we persuade, bribe, or coerce a group of participants to make them act in a way that will motivate the rest of the players to act accordingly to the desired equilibrium. Formally, we ask which subset of the players can adopt the goal equilibrium strategies that will make acting according to the desired equilibrium a best response for the other players. We call such a subset a direct control set, prove some connections to strength of equilibrium, and study the hardness to find such lightest sets, even approximately. We then solve important subcases and provide approximation algorithms, assuming monotonicity. Next, we concentrate on potential games and prove that, while the problem of finding such a set is \NP-hard, even for constant-factor approximation, we can still solve the problem approximately or even precisely in relevant special cases. We approximately solve this problem for singleton potential games and treat more closely specific potential games, such as symmetric games and coordination games on graphs.

==> graph_game.tex <==
\section{Graphical Games}\label{Sec:graph_game}
